Preprocessing in Inductive Logic Programming

Inductive logic programming is a type of machine learning in which logic programs are learned from examples. This learning typically occurs relative to some background knowledge provided as a logic program. This dissertation introduces bottom preprocessing, a method for generating initial constraints on the programs an ILP system must consider. Bottom preprocessing applies ideas from inverse entailment to modern ILP systems. Inverse entailment is an influential early ILP approach introduced with Progol. This dissertation also presents $\bot$-Popper, an implementation of bottom preprocessing for the modern ILP system Popper. It is shown experimentally that bottom preprocessing can reduce learning times of ILP systems on hard problems. This reduction can be especially significant when the amount of background knowledge in the problem is large.

==> old/introduction.tex <==
\chapter{Introduction}
Since the early days of artificial intelligence research, researchers have been interested in creating computer programs which write other computer programs. \cite{friedman1963alonzo, simon1963experiments} This problem is called program synthesis and it remains challenging to this day. Recently, massive neural networks like GPT-3, when customized to coding problems, have captured media attention and birthed commercial products. These customized deep learning models are capable of generating sophisticated program fragments from code comments.\cite{chen2021evaluating} \todo{Read the paper more thoroughly. Cite more.} While high visibility, this is only one of many exciting approaches to program synthesis under active research.
\ac{I would cut almost everything in this paragraph. Talking about NNs and GPT-3 is a slightly weird way to start your thesis. You can start by talking about program synthesis but just say "there are many approaches such as using genetic programming \cite{}, NNs \cite{}
, etc}.

In this dissertation, we \ac{in your thesis, I would say 'I' rather than 'We' as it is all your comntribution} will focus on a different, logic based approach to program synthesis called \emph{inductive logic programming} (ILP). ILP systems are machine learning algorithms which take as input a set of examples and a logic program constituting background knowledge. They produce a logic program which, when coupled with the background knowledge, covers all positive examples and does not cover any negative examples. 

Intutively, we can think of the background knowledge as a library of helper relations which describe what we know about the problem domain. The examples are then the specification for what we expect the program to do. Viewed this way, ILP systems use the library to generate a program which perfectly matches the specification. There is an interesting parallel to test driven development (TDD), a methodology in which developers write tests before filling in an implementation that passes the tests.\todo{(Cite TDD? Worth cutting?)} With ILP, the software writes the implementation.
\ac{yes, cute}

\section{Advantages and disadvantages of ILP}
Inductive logic programming has several advantages over other approaches to program synthesis:
\begin{enumerate}
    \item It usually requires very few examples to learn a program successfully. This stands in constrast to deep learning approaches which are frequently very data hungry.
    \item The output of an ILP system is a human readable program with strong logical properties.
    \item The learning process is based on logic and is often deterministic. This means intermediate results can be easily debugged and understood. 
    \item ILP supports transfer learning. The program produced for one ILP problem can serve as background knowledge for further learning. This ability to compose ILP problems is very desirable when learning complex systems. 
\end{enumerate}

\todo{I think the above claims are fine. I'd like to read some of the references in the ILP at 30 paper when I have time. Then I'll update these with citations and rework the language to be more in line with the cited papers.}

The main disadvantage of ILP systems is that they tend to search a very large hypothesis space. The space of possible programs is vast. For many programming languages \ac{this statement is a bit imprecise as ILP focuses on logic programming, so there are no other programming languages. You might want to say something along the lines of ILP systems usually induce first-order programs and then go on to briefly state why this expressivity is so challenging (undecidable, infinite domains, etc)}, it can even be infinite. \todo{Clean up. Reference.} Many ILP systems will exhaustively search these spaces \ac{that is not true}. Most ILP systems thus focus on pruning these very large hypothesis spaces as they search them efficiently. 

\ac{there are a lot of dubious claims above. You need to justify anything that is not self-evident}

The simplest method ILP systems use to constrain the hypothesis space is with a language bias. \ac{this statement needs more nuance. All forms of ML need an inductive bias, such as the neural architecture in a NNs, as without it ML is futile (Tom Mitchell, ML book). In ILP, a key form of inductive bias is the langiuage bias}. The language bias defines the predicates available for use in a program. The bias can also include meta-information about types as well as \todo{language restrictions}. At its most basic level, the language bias ensures an ILP system doesn't \ac{does not} need to try every possible string \ac{what is a string?} as a potential predicate.

In chapter 2, we'll \ac{we will} discuss a variety of approaches that modern ILP systems use to minimize their search space. In this dissertation, we introduce preprocessing as a new way to reduce the search space for ILP systems.

\section{The Trains Problem}
\begin{example}
\label{trains_example}
To explain ILP, we give an example of a classic problem in machine learning, Michalski's train problem.\cite{larson1977inductive} Figure \ref{trains} shows four trains taken from a machine learning competition held in 1994.\cite{michie1994international} Trains \texttt{t1} and \texttt{t2} are westbound, facing left, while \texttt{t3} and \texttt{t4} are eastbound, facing right. Suppose we would like to find a relation \texttt{f} which holds for eastbound trains but not for westbound trains \ac{I would say a relation f(Train) which ....}.

\begin{figure}
\label{trains}
\centering
\includegraphics[width=0.9\textwidth]{trains_figure}
\caption{Examples from the Michalski trains problem.}
\end{figure}

Since this problem is simple, the reader might be able to find a solution with a quick visual inspection.  All eastbound trains have a car carrying a rectangular load while none of the westbound cars carry a rectangular load. It should be clear, however, that with more trains this problem quickly becomes difficult to solve. ILP systems can easily solve most trains problems involving five eastbound and westbound trains. We show in chapter 6 that the preprocessing technique introduced in this dissertation increases the frequency with which a modern ILP system can find solutions involving 20 examples of each type of train. \todo{Update  this in the experiments once that part is written/done?}

To make the problem solvable by an ILP system, we encode the information in the images as facts in a logic programming language. We might choose to represent train \texttt{t3} in the following way:
\ac{refer to the figure using ref{figure}. Avoid using relative positioning.}


\begin{figure}[h]
\begin{multicols}{2}
\begin{lstlisting}
train(t3).
has_car(t3, t3_c1).
has_car(t3, t3_c2).
short(t3_c1).
short(t3_c2).
two_wheels(t3_c1).
two_wheels(t3_c2).
roof_open(t3_c1).
roof_open(t3_c2).
has_load(t3_c1, t3_c1_l1).
has_load(t3_c2, t3_c2_l1).
triangle(t3_c1_l1).
rectangle(t3_c2_l1).
\end{lstlisting}
\end{multicols}
\caption{Logic encoding for train \texttt{t3}.}
\end{figure}

Taking a similar approach for trains \texttt{t1}, \texttt{t2}, and \texttt{t4}, we can produce a full logic program. This program is our background knowledge. Our positive examples are $\{\texttt{f(t3)}, \texttt{f(t4)} \}$ and our negative examples are $\{\texttt{f(t1)}, \texttt{f(t2)}\}$. Given this background knowledge and these examples, an ILP system learns the following logic program, $H$, which matches our intuitive solution:

\begin{lstlisting}
f(A) :- has_car(A, B), has_load(B, C), rectangle(C).
\end{lstlisting}

\end{example}

\section{Progol and Popper}
\ac{this section is far too brief. It will be far to difficult for a reader or asessor to understand}
The techniques an ILP system uses to discover a program like $H$ can vary. The influential early ILP system Progol\cite{muggleton1995inverse} relies on a concept called the bottom clause. The bottom clause of an example is the most specific clause which, relative to the background knowledge, entails the example. Thus any clause which entails the bottom clause relative to the background knowledge must also entail the example. 

Given background knowledge $B$ as described above, the bottom clause of \lstinline|f(t3)|, $\bot_B(e)$, is: 

\begin{lstlisting}
f(A) :- 
    train(A), has_car(A,B), @\textbf{has\_car(A,C)}@,
    short(B), two_wheels(B), roof_open(B),
    short(C), two_wheels(C), roof_open(C),
    has_load(B,D), @\textbf{has\_load(C,E)}@, triangle(D), @\textbf{rectangle(E)}@.
\end{lstlisting}

Checking entailment between clauses is undecidable. \todo{Cite. Church?} For this reason, Progol instead tests $\theta$-subsumption, which we define more precisely in chapter 3. Our solution $H$ subsumes $\bot_B(e)$ because there is a substitution $\theta = \{C/B, E/C\}$, such that $H\theta \subseteq \bot(e)$. Specifically, $H\theta$ is:

\begin{lstlisting}
f(A) :- has_car(A, C), has_load(C, E), rectangle(E).
\end{lstlisting}

The literals in $H\theta$ are the bolded literals in $\bot_B(e)$. This process of finding clauses which subsume the bottom clause of an example is called bottom generalization.\cite{ray2003hybrid} We describe Progol's search mechanism and bottom generalization in more detail in chapter 2.

The modern, meta-level ILP system Popper \cite{cropper2021learning} uses a very different approach. It encodes the ILP problem as a constraint satisfaction problem on the syntax of logic programming. It uses a generate-test-constrain loop. In each loop:

\begin{enumerate}
    \item The CSP produces a hypothesis program.
    \item Popper tests that program against the examples.
    \item If the program fails, Popper generates constraints on future hypotheses
\end{enumerate}

For the trains problem above, Popper might produce the hypothesis

\begin{lstlisting}
f(A) :- has_car(A, B), two_wheels(B).
\end{lstlisting}

This hypothesis covers both positive examples, \lstinline|f(t3)| and \lstinline|f(t4)|. However, it also covers the negative examples \lstinline|f(t1)| and \lstinline|f(t2)| since all four trains have a car with two wheels. Popper concludes that any clause containing \lstinline|has_car(A, B),| \lstinline|two_wheels(B)| will cover a negative example. It prunes any hypothesis containing a clause with those literals from the hypothesis space. We also discuss Popper in more detail in chapter 2.

\todo{Include the figure showing the generate-test-constrain loop in Popper}

\section{Preprocessing}
Popper has shown significant speedups over earlier ILP systems on a range of ILP problems. Despite being faster on average, Popper's approach is still compatible with Progol's bottom clause. Popper only learns from the examples and background knowledge when it tests a hypothesis. Progol, on the other hand, first computes the bottom clause using only the examples and BK before running its  search. 

In this dissertation we examine how we can use information derived from the background knowledge and examples to reduce the size of Popper's initial hypothesis space. Using ideas from Progol, we notice that a hypothesis can be pruned from Popper's hypothesis space if:
\begin{enumerate}
    \item the hypothesis entails the bottom clause of some negative example.
    \item the hypothesis does not entail the bottom clause of some positive example.
\end{enumerate}

Popper can take as input a set of hypothesis constraints which apply directly to its CSP encoding. In order to prune Popper's search space according to the ideas above, we convert the bottom clauses into hypothesis constraints that Popper's CSP solver can use. This dissertation demonstrates the effectiveness of this approach.

Popper has the desirable property that it finds optimal solutions if they exist. Progol cannot guarantee optimality due to its reliance on $\theta$-subsumption as an approximation of entailment. Preprocessing also relies on $\theta$-subsumption. We show that we can maintain Popper's guarantee of optimality when we generate constraints from negative examples. However, once we use positive examples, we are forced to sacrifice optimality.

\paragraph{Contributions}
Specifically, this dissertation makes the following contributions:

\begin{enumerate}
    \item We demonstrate that preprocessing hypothesis constraints can be used to prune the hypothesis space of meta-level ILP systems.
    \item We show that hypothesis constraints derived with bottom generalization using $\theta$-subsumption: 
        \begin{enumerate}
            \item do not prune solutions when generated from negative examples.
            \item can prune solutions when generated from positive examples.
        \end{enumerate}
    \item We describe a working implementation of preprocessing for Popper based on bottom generalization.
    \item We test a variety of hypothesis constraints derived from bottom clauses and show their effect on performance.
    \item We show that preprocessing improves the runtime of Popper on a variety of difficult ILP problems.
\end{enumerate}

\section{Outline}
\begin{itemize}
    \item In chapter 2, we describe Progol and Popper in more detail. We compare other similar ILP systems. We discuss similarities between preprocessing and approaches taken in other systems such as NRSample and FastLAS.
    \item In chapter 3, we review logic programming, precisely define the ILP problem input, and provide supporting definitions of subsumption and generalization.
    \item In chapter 4, we prove soundness for preprocessing constraints generated from negative example bottom clauses. We show that constraints from positive example bottom clauses are not sound but do not prune all solutions. We show that we can loosen our definitions of generalization in certain ways without affecting these results.
    \item In chapter 5, we describe how we implemented preprocessing for Popper and prove the correctness of our approach.
    \item In chapter 6, we give experimental proof that preprocessing both prunes hypotheses and improves runtime for many ILP problems. We also compare the improvements gained from different types of constraints derived with bottom generalization.
    \item Finally, in chapter 7, we explain the limitations of preprocessing in ILP and discuss possible future work that could be done on the topic.
\end{itemize}

\todo{I'm a bit concerned this introduction is too long. I'm open to suggestions for parts I shouldn't bother explaining until their chapter.}


\todo{Version 2 stuff}
To demonstrate both inductive logic programming and preprocessing, we give an example using a classic machine learning problem.

\begin{example}
\label{trains_example}
Michalski's train problem \cite{larson1977inductive} will serve as a running example throughout this dissertation. Figure \ref{fig:trains_image} shows four example trains.Trains \texttt{t1} and \texttt{t2} are westbound, facing left, while \texttt{t3} and \texttt{t4} are eastbound, facing right. Suppose we would like to find a relation \texttt{f(Train)} which holds for eastbound trains but not for westbound trains. Finding such a relation was the basis of a machine learning competition held in 1994 and from which these images were  taken.\cite{michie1994international} 

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{trains_figure}
\caption{Examples from the Michalski trains problem.}
\label{fig:trains_image}
\end{figure}

\todo{Delete all this and use a different problem with more trains. Or switch to something else.  Since this problem is simple, the reader might be able to find a solution with a quick visual inspection.  All eastbound trains have a car carrying a rectangular load while none of the westbound cars carry a rectangular load. It should be clear, however, that with more trains this problem quickly becomes difficult to solve. ILP systems can easily solve most trains problems involving five eastbound and westbound trains. We show in chapter 6 that the preprocessing technique introduced in this dissertation increases the frequency with which a modern ILP system can find solutions involving 20 examples of each type of train.}

\begin{figure}
\begin{multicols}{2}
\begin{lstlisting}
train(t3).
has_car(t3, t3_c1).
has_car(t3, t3_c2).
short(t3_c1).
short(t3_c2).
two_wheels(t3_c1).
two_wheels(t3_c2).
roof_open(t3_c1).
roof_open(t3_c2).
has_load(t3_c1, t3_c1_l1).
has_load(t3_c2, t3_c2_l1).
triangle(t3_c1_l1).
rectangle(t3_c2_l1).
\end{lstlisting}
\end{multicols}
\caption{Logic program for train \texttt{t3}.}
\label{fig:trains_logic}
\end{figure}

In order for an ILP system to solve this problem, the information in the image must be written in a logic programming language. Train \texttt{t3} could be represented using the code in Figure \ref{fig:trains_logic} \todo{Figure ref not working.} Taking a similar approach for trains \texttt{t1}, \texttt{t2}, and \texttt{t4} produces a full logic program which constitutes the background knowledge, $B$, for this instance of the trains problem. The positive examples are $\{\texttt{f(t3)}, \texttt{f(t4)} \}$ and the negative examples are $\{\texttt{f(t1)}, \texttt{f(t2)}\}$. Given this background knowledge and these examples, an ILP system learns the following logic program, $H$:

\begin{lstlisting}
f(A) :- has_car(A, B), has_load(B, C), rectangle(C).
\end{lstlisting}

The bottom clause of the positive example $e = \lstinline|f(t3)|$ relative to $B$, $\bot_B(e)$, is as follows: 

\begin{lstlisting}
f(A) :- 
    train(A), has_car(A,B), has_car(A,C),
    short(B), two_wheels(B), roof_open(B),
    short(C), two_wheels(C), roof_open(C),
    has_load(B,D), has_load(C,E), triangle(D), rectangle(E).
\end{lstlisting}

\todo{Fill in examples of preprocessing.}
\end{example}

\begin{lstlisting}
palindrome(A) :- first(A,B), last(A,B), middle(A,C), length(A,F), first(C,G), last(C,G), length(C,I), middle(C,E), empty(E), length(E,H), one(D).
\end{lstlisting}
